Towards Neuromorphic Processing for Next-Generation MU-MIMO Detection

Upcoming physical layer (PHY) processing solutions, leveraging multiple-input multiple-output (MIMO) advances, are expected to support broad transmission bandwidths and the concurrent transmission of multiple information streams. However, the inherent computational complexities of conventional MIMO PHY algorithms pose significant practical challenges, not only in meeting the strict real-time processing latency requirements but also in maintaining practical computational power consumption budgets. Novel computing paradigms, such as neuromorphic computing, promise substantial gains in computational power efficiency. However, it is unknown whether it is feasible or efficient to realize practical PHY algorithms on such platforms. In this work, we evaluate for the first time the potential of neuromorphic computing principles for multi-user (MU)-MIMO detection. In particular, we developed the first spiking-based MU-MIMO simulator that meets practical error-rate targets, suggesting power gains of at least one order of magnitude when realized on actual neuromorphic hardware, compared to conventional processing platforms. Finally, we discuss the challenges and future research directions that could unlock practical neuromorphic-based MU-MIMO systems and revolutionize PHY power efficiency.

==> 7_related_work.tex <==


The second common approach are a category of heuristic and metaheuristic approaches like simulated annealing and tabu file:///C:/Users/george/Downloads/4589.pdf search where they have shown 
Heuristic methods, including simulated annealing and tabu search, are more computationally efficient than exhaustive search yet pose challenges for real-time performance. While they do not guarantee achieving the global minimum, their time complexity is influenced by the complexity of the optimization problem and necessitates multiple evaluations of the objective function.

Quantum approaches, while they have shown promising perfromance , due to their high computational power costs , their advantage over conventional approaches in MIMO detection appears either  in unrealisticly large MIMO dimensions and bandwidths that other practical challenges such as (scheduling,resource allocation..)  prohibit their application.


More recently, neuromorphic approaches based on spiking neural networks have been discussed to solve QUBO problems, with , to the best of our knowledge no existing evaluation on MIMO detection systems.
The core principle of existing neuromorphic qubo solvers is to map the QUBO matrix as a graph of interconnected neurons, (a spiking neural network) that given some arbitrary stimuli and allowing it to evolve , the neural dynamics allow it to converge to a minima for the QUBO problem. Have been examined in the context of sparse arrays, without an evaluation on whether it makes sense for MIMO [put all the references I have for spikingQUBO]
As we will also discuss in Section X , each neuron integrates.. and emits a spike ... based on the spiking rate a solution for the qubo problem can be decoded. Their event driven nature, as well as the very simple neuron design allows for substantial power gains. Additional benefits from this approach is the alleviation of memory related bottlenecks that have been longstanding in the von neuman architectures as well as their massive parallelization capabilities and their inherited scalability. Still to the best of our knowledge this is the first time that aspects of neuromorphic computing has  been discussed in the context of MIMO and massive MIMO. 

% For the rest of the systems variables we analyzed 
% Discuss briefly the changes versus the number of iterations




% \textit{SIMULATION PARAMETERS TABLE
% }For our simulation, we selected an R value of 1 and a Dt/tau at 0.01. For the initial I(0) values we investigated multiple \gls{qubo} matrices and found out the 99th percentile of the examined \gls{qubo} matrices reached their minimum energy state when I(0) was in the range of [x to X]. Due to the wide range of distribution we 

% to reasonably balance the number of parallel networks for each matrix we investigated 10 points within this interval the results of which are presented in Section X..


% Running Experiments
% \begin{itemize}
%     \item I
%     \item tau
%     \item vth
%     \item Simul Time (iters)
% \end{itemize}




% % \begin{figure}
% %     \centering
% %     \includegraphics{Figures/ber_vs_I.png}
% %     \caption{Average BER for different initial I values (comm ,SNR HAD NOT EFFECT, constant scaling also no effect, execution time has effect see dnload pic)}
% %     \label{fig:enter-label2}
% % \end{figure}

% add graph with the tau (small values) 
% add graph with the 


% % \begin{figure}
% %     \centering
% %     \includegraphics{Figures/ber_vs_tau.png}
% %     \caption{Caption}
% %     \label{fig:enter-label3}
% % \end{figure}



% \section{Spiking Neuron Approach (with and without stochastic input)}
% new experiment for time to solution
% General gains :
%  absence of matrix inversions that have large complexity and not very good parallelization properties this is particularly important for large MU-MIMO systems with many users and antennas.
%  This has immediate effect on power (can we discuss this?) 
%  and processing latency, estimate a speedup
%  and system scalability compared to a conventional system architecture
%  a true north neuron required approximately X gates, per neuron (how much on an FPGA ?)
 
% discussion:
% no stoch = more sensitive to the initial conditions
% similar performance in cases better than linear appraoches (better than ZF , similar to MMSE)
% potential for complexity gains
% require metric evaluations but those are simple additions 
% variations that improve perfromance (annealing approach -> starting from an already good solution , reducing noise gradually, stopping noise at the half of the simulation)
% extracting the correct solution : 
% >best out of all states (not efficient)
% >majority vote (very hardware friendly, maj-vote based on the last half)
% >can we discuss anything about LLRS?
% challenges for higher constellations 

% \section{Greedy Deterministic Approach}
% works for  massive \gls{mimo}
% The employed neuron model is simplified as such  ..
% Starting from a high initial potential neurons update their values based on the summation of rows of the qubo matrix, since there is no stochastic input into the system the inhibitory neurons will start declining, the first neuron to stop spiking will be the ones who correspond to the most negative line on the qubo matrix, the corresponding bit will be assigned the value 0. This will reduce the dimensionality of the problem by 1, the process will continue with the updated values..
% discussion : greedy approach -> performance similar to algorithms such as ..





% \section{Results}
% Discuss way forward
% discuss accelerators challenges for neuromorphic accelerators
% the gains that we dont have to update the whole matrix

% \begin{itemize}
%     \item Discuss scalability
%     \item Disucss energy (\url{https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=7966350} very simple)
% \end{itemize}

==> 8_conclusions.tex <==
In this work we developped a first spiking based MU-MIMO detector, showing that neuromorphic computing has the potential to reach practical BER targets of modern communications systems while delivering substantial power consumption gains from the computational part. Moreover we discussed the challenges and the future directions that can truly revolutionize next generation PHY developements.
